Transverse spin-dependent azimuthal correlations of charged pion pairs measured in p$^\uparrow$+p collisions at $\sqrt{s}$ = 500 GeV

The transversity distribution, which describes transversely polarized quarks in transversely polarized nucleons, is a fundamental component of the spin structure of the nucleon, and is only loosely constrained by global fits to existing semi-inclusive deep inelastic scattering (SIDIS) data. In transversely polarized $p^\uparrow+p$ collisions it can be accessed using transverse polarization dependent fragmentation functions which give rise to azimuthal correlations between the polarization of the struck parton and the final state scalar mesons. This letter reports on spin dependent di-hadron correlations measured by the STAR experiment. The new dataset corresponds to 25 pb$^{-1}$ integrated luminosity of $p^\uparrow+p$ collisions at $\sqrt{s}=500$ GeV, an increase of more than a factor of ten compared to our previous measurement at $\sqrt{s}=200$ GeV. Non-zero asymmetries sensitive to transversity are observed at a $Q^2$ of several hundred GeV and are found to be consistent with the former measurement and a model calculation. %we observe consistent with the former measurement are observed.} We expect that these data will enable an extraction of transversity with comparable precision to current SIDIS datasets but at much higher momentum transfers where subleading effects are suppressed.

==> authorList.tex <==
\affiliation{AGH University of Science and Technology, FPACS, Cracow 30-059, Poland}
\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}
\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\affiliation{University of California, Berkeley, California 94720}
\affiliation{University of California, Davis, California 95616}
\affiliation{University of California, Los Angeles, California 90095}
\affiliation{Central China Normal University, Wuhan, Hubei 430079}
\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\affiliation{Creighton University, Omaha, Nebraska 68178}
\affiliation{Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\affiliation{Nuclear Physics Institute AS CR, 250 68 Prague, Czech Republic}
\affiliation{Frankfurt Institute for Advanced Studies FIAS, Frankfurt 60438, Germany}
\affiliation{Institute of Physics, Bhubaneswar 751005, India}
\affiliation{Indiana University, Bloomington, Indiana 47408}
\affiliation{Alikhanov Institute for Theoretical and Experimental Physics, Moscow 117218, Russia}
\affiliation{University of Jammu, Jammu 180001, India}
\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\affiliation{Kent State University, Kent, Ohio 44242}
\affiliation{University of Kentucky, Lexington, Kentucky 40506-0055}
\affiliation{Lamar University, Physics Department, Beaumont, Texas 77710}
\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000}
\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\affiliation{Lehigh University, Bethlehem, Pennsylvania 18015}
\affiliation{Max-Planck-Institut fur Physik, Munich 80805, Germany}
\affiliation{Michigan State University, East Lansing, Michigan 48824}
\affiliation{National Research Nuclear University MEPhI, Moscow 115409, Russia}
\affiliation{National Institute of Science Education and Research, HBNI, Jatni 752050, India}
\affiliation{National Cheng Kung University, Tainan 70101 }
\affiliation{Ohio State University, Columbus, Ohio 43210}
\affiliation{Institute of Nuclear Physics PAN, Cracow 31-342, Poland}
\affiliation{Panjab University, Chandigarh 160014, India}
\affiliation{Pennsylvania State University, University Park, Pennsylvania 16802}
\affiliation{Institute of High Energy Physics, Protvino 142281, Russia}
\affiliation{Purdue University, West Lafayette, Indiana 47907}
\affiliation{Pusan National University, Pusan 46241, Korea}
\affiliation{Rice University, Houston, Texas 77251}
\affiliation{Rutgers University, Piscataway, New Jersey 08854}
\affiliation{Universidade de Sao Paulo, Sao Paulo, Brazil, 05314-970}
\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\affiliation{Shandong University, Jinan, Shandong 250100}
\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\affiliation{State University of New York, Stony Brook, New York 11794}
\affiliation{Temple University, Philadelphia, Pennsylvania 19122}
\affiliation{Texas A\&M University, College Station, Texas 77843}
\affiliation{University of Texas, Austin, Texas 78712}
\affiliation{University of Houston, Houston, Texas 77204}
\affiliation{Tsinghua University, Beijing 100084}
\affiliation{University of Tsukuba, Tsukuba, Ibaraki, Japan,305-8571}
\affiliation{Southern Connecticut State University, New Haven, Connecticut 06515}
\affiliation{University of California, Riverside, California 92521}
\affiliation{United States Naval Academy, Annapolis, Maryland 21402}
\affiliation{Valparaiso University, Valparaiso, Indiana 46383}
\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\affiliation{Wayne State University, Detroit, Michigan 48201}
\affiliation{World Laboratory for Cosmology and Particle Physics (WLCAPP), Cairo 11571, Egypt}
\affiliation{Yale University, New Haven, Connecticut 06520}
\author{L.~Adamczyk}\affiliation{AGH University of Science and Technology, FPACS, Cracow 30-059, Poland}
\author{J.~R.~Adams}\affiliation{Ohio State University, Columbus, Ohio 43210}
\author{J.~K.~Adkins}\affiliation{University of Kentucky, Lexington, Kentucky 40506-0055}
\author{G.~Agakishiev}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{M.~M.~Aggarwal}\affiliation{Panjab University, Chandigarh 160014, India}
\author{Z.~Ahammed}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{N.~N.~Ajitanand}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{I.~Alekseev}\affiliation{Alikhanov Institute for Theoretical and Experimental Physics, Moscow 117218, Russia}\affiliation{National Research Nuclear University MEPhI, Moscow 115409, Russia}
\author{D.~M.~Anderson}\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{R.~Aoyama}\affiliation{University of Tsukuba, Tsukuba, Ibaraki, Japan,305-8571}
\author{A.~Aparin}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{D.~Arkhipkin}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{E.~C.~Aschenauer}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{M.~U.~Ashraf}\affiliation{Tsinghua University, Beijing 100084}
\author{A.~Attri}\affiliation{Panjab University, Chandigarh 160014, India}
\author{G.~S.~Averichev}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{X.~Bai}\affiliation{Central China Normal University, Wuhan, Hubei 430079}
\author{V.~Bairathi}\affiliation{National Institute of Science Education and Research, HBNI, Jatni 752050, India}
\author{K.~Barish}\affiliation{University of California, Riverside, California 92521}
\author{A.~Behera}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{R.~Bellwied}\affiliation{University of Houston, Houston, Texas 77204}
\author{A.~Bhasin}\affiliation{University of Jammu, Jammu 180001, India}
\author{A.~K.~Bhati}\affiliation{Panjab University, Chandigarh 160014, India}
\author{P.~Bhattarai}\affiliation{University of Texas, Austin, Texas 78712}
\author{J.~Bielcik}\affiliation{Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\author{J.~Bielcikova}\affiliation{Nuclear Physics Institute AS CR, 250 68 Prague, Czech Republic}
\author{L.~C.~Bland}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{I.~G.~Bordyuzhin}\affiliation{Alikhanov Institute for Theoretical and Experimental Physics, Moscow 117218, Russia}
\author{J.~Bouchet}\affiliation{Kent State University, Kent, Ohio 44242}
\author{J.~D.~Brandenburg}\affiliation{Rice University, Houston, Texas 77251}
\author{A.~V.~Brandin}\affiliation{National Research Nuclear University MEPhI, Moscow 115409, Russia}
\author{D.~Brown}\affiliation{Lehigh University, Bethlehem, Pennsylvania 18015}
\author{J.~Bryslawskyj}\affiliation{University of California, Riverside, California 92521}
\author{I.~Bunzarov}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{J.~Butterworth}\affiliation{Rice University, Houston, Texas 77251}
\author{H.~Caines}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{M.~Calder{\'o}n~de~la~Barca~S{\'a}nchez}\affiliation{University of California, Davis, California 95616}
\author{J.~M.~Campbell}\affiliation{Ohio State University, Columbus, Ohio 43210}
\author{D.~Cebra}\affiliation{University of California, Davis, California 95616}
\author{I.~Chakaberia}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{P.~Chaloupka}\affiliation{Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\author{Z.~Chang}\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{N.~Chankova-Bunzarova}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{A.~Chatterjee}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{S.~Chattopadhyay}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{X.~Chen}\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000}
\author{J.~H.~Chen}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{X.~Chen}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{J.~Cheng}\affiliation{Tsinghua University, Beijing 100084}
\author{M.~Cherney}\affiliation{Creighton University, Omaha, Nebraska 68178}
\author{W.~Christie}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{G.~Contin}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{H.~J.~Crawford}\affiliation{University of California, Berkeley, California 94720}
\author{S.~Das}\affiliation{Central China Normal University, Wuhan, Hubei 430079}
\author{T.~G.~Dedovich}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{J.~Deng}\affiliation{Shandong University, Jinan, Shandong 250100}
\author{A.~A.~Derevschikov}\affiliation{Institute of High Energy Physics, Protvino 142281, Russia}
\author{L.~Didenko}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{C.~Dilks}\affiliation{Pennsylvania State University, University Park, Pennsylvania 16802}
\author{X.~Dong}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{J.~L.~Drachenberg}\affiliation{Lamar University, Physics Department, Beaumont, Texas 77710}
\author{J.~E.~Draper}\affiliation{University of California, Davis, California 95616}
\author{J.~C.~Dunlop}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{L.~G.~Efimov}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{N.~Elsey}\affiliation{Wayne State University, Detroit, Michigan 48201}
\author{J.~Engelage}\affiliation{University of California, Berkeley, California 94720}
\author{G.~Eppley}\affiliation{Rice University, Houston, Texas 77251}
\author{R.~Esha}\affiliation{University of California, Los Angeles, California 90095}
\author{S.~Esumi}\affiliation{University of Tsukuba, Tsukuba, Ibaraki, Japan,305-8571}
\author{O.~Evdokimov}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\author{J.~Ewigleben}\affiliation{Lehigh University, Bethlehem, Pennsylvania 18015}
\author{O.~Eyser}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{R.~Fatemi}\affiliation{University of Kentucky, Lexington, Kentucky 40506-0055}
\author{S.~Fazio}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{P.~Federic}\affiliation{Nuclear Physics Institute AS CR, 250 68 Prague, Czech Republic}
\author{P.~Federicova}\affiliation{Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\author{J.~Fedorisin}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{Z.~Feng}\affiliation{Central China Normal University, Wuhan, Hubei 430079}
\author{P.~Filip}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{E.~Finch}\affiliation{Southern Connecticut State University, New Haven, Connecticut 06515}
\author{Y.~Fisyak}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{C.~E.~Flores}\affiliation{University of California, Davis, California 95616}
\author{J.~Fujita}\affiliation{Creighton University, Omaha, Nebraska 68178}
\author{L.~Fulek}\affiliation{AGH University of Science and Technology, FPACS, Cracow 30-059, Poland}
\author{C.~A.~Gagliardi}\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{F.~Geurts}\affiliation{Rice University, Houston, Texas 77251}
\author{A.~Gibson}\affiliation{Valparaiso University, Valparaiso, Indiana 46383}
\author{M.~Girard}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{D.~Grosnick}\affiliation{Valparaiso University, Valparaiso, Indiana 46383}
\author{D.~S.~Gunarathne}\affiliation{Temple University, Philadelphia, Pennsylvania 19122}
\author{Y.~Guo}\affiliation{Kent State University, Kent, Ohio 44242}
\author{A.~Gupta}\affiliation{University of Jammu, Jammu 180001, India}
\author{W.~Guryn}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{A.~I.~Hamad}\affiliation{Kent State University, Kent, Ohio 44242}
\author{A.~Hamed}\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{A.~Harlenderova}\affiliation{Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\author{J.~W.~Harris}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{L.~He}\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{S.~Heppelmann}\affiliation{Pennsylvania State University, University Park, Pennsylvania 16802}
\author{S.~Heppelmann}\affiliation{University of California, Davis, California 95616}
\author{A.~Hirsch}\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{S.~Horvat}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{B.~Huang}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\author{X.~ Huang}\affiliation{Tsinghua University, Beijing 100084}
\author{T.~Huang}\affiliation{National Cheng Kung University, Tainan 70101 }
\author{H.~Z.~Huang}\affiliation{University of California, Los Angeles, California 90095}
\author{T.~J.~Humanic}\affiliation{Ohio State University, Columbus, Ohio 43210}
\author{P.~Huo}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{G.~Igo}\affiliation{University of California, Los Angeles, California 90095}
\author{W.~W.~Jacobs}\affiliation{Indiana University, Bloomington, Indiana 47408}
\author{A.~Jentsch}\affiliation{University of Texas, Austin, Texas 78712}
\author{J.~Jia}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{K.~Jiang}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{S.~Jowzaee}\affiliation{Wayne State University, Detroit, Michigan 48201}
\author{E.~G.~Judd}\affiliation{University of California, Berkeley, California 94720}
\author{S.~Kabana}\affiliation{Kent State University, Kent, Ohio 44242}
\author{D.~Kalinkin}\affiliation{Indiana University, Bloomington, Indiana 47408}
\author{K.~Kang}\affiliation{Tsinghua University, Beijing 100084}
\author{D.~Kapukchyan}\affiliation{University of California, Riverside, California 92521}
\author{K.~Kauder}\affiliation{Wayne State University, Detroit, Michigan 48201}
\author{H.~W.~Ke}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{D.~Keane}\affiliation{Kent State University, Kent, Ohio 44242}
\author{A.~Kechechyan}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{Z.~Khan}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\author{D.~P.~Kiko\l{}a~}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{C.~Kim}\affiliation{University of California, Riverside, California 92521}
\author{I.~Kisel}\affiliation{Frankfurt Institute for Advanced Studies FIAS, Frankfurt 60438, Germany}
\author{A.~Kisiel}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{L.~Kochenda}\affiliation{National Research Nuclear University MEPhI, Moscow 115409, Russia}
\author{M.~Kocmanek}\affiliation{Nuclear Physics Institute AS CR, 250 68 Prague, Czech Republic}
\author{T.~Kollegger}\affiliation{Frankfurt Institute for Advanced Studies FIAS, Frankfurt 60438, Germany}
\author{L.~K.~Kosarzewski}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{A.~F.~Kraishan}\affiliation{Temple University, Philadelphia, Pennsylvania 19122}
\author{L.~Krauth}\affiliation{University of California, Riverside, California 92521}
\author{P.~Kravtsov}\affiliation{National Research Nuclear University MEPhI, Moscow 115409, Russia}
\author{K.~Krueger}\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}
\author{N.~Kulathunga}\affiliation{University of Houston, Houston, Texas 77204}
\author{L.~Kumar}\affiliation{Panjab University, Chandigarh 160014, India}
\author{J.~Kvapil}\affiliation{Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\author{J.~H.~Kwasizur}\affiliation{Indiana University, Bloomington, Indiana 47408}
\author{R.~Lacey}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{J.~M.~Landgraf}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{K.~D.~ Landry}\affiliation{University of California, Los Angeles, California 90095}
\author{J.~Lauret}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{A.~Lebedev}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{R.~Lednicky}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{J.~H.~Lee}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{W.~Li}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{Y.~Li}\affiliation{Tsinghua University, Beijing 100084}
\author{X.~Li}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{C.~Li}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{J.~Lidrych}\affiliation{Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\author{T.~Lin}\affiliation{Indiana University, Bloomington, Indiana 47408}
\author{M.~A.~Lisa}\affiliation{Ohio State University, Columbus, Ohio 43210}
\author{P.~ Liu}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{H.~Liu}\affiliation{Indiana University, Bloomington, Indiana 47408}
\author{F.~Liu}\affiliation{Central China Normal University, Wuhan, Hubei 430079}
\author{Y.~Liu}\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{T.~Ljubicic}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{W.~J.~Llope}\affiliation{Wayne State University, Detroit, Michigan 48201}
\author{M.~Lomnitz}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{R.~S.~Longacre}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{S.~Luo}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\author{X.~Luo}\affiliation{Central China Normal University, Wuhan, Hubei 430079}
\author{L.~Ma}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{G.~L.~Ma}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{Y.~G.~Ma}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{R.~Ma}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{N.~Magdy}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{R.~Majka}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{D.~Mallick}\affiliation{National Institute of Science Education and Research, HBNI, Jatni 752050, India}
\author{S.~Margetis}\affiliation{Kent State University, Kent, Ohio 44242}
\author{C.~Markert}\affiliation{University of Texas, Austin, Texas 78712}
\author{H.~S.~Matis}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{D.~Mayes}\affiliation{University of California, Riverside, California 92521}
\author{K.~Meehan}\affiliation{University of California, Davis, California 95616}
\author{J.~C.~Mei}\affiliation{Shandong University, Jinan, Shandong 250100}
\author{Z.~ W.~Miller}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\author{N.~G.~Minaev}\affiliation{Institute of High Energy Physics, Protvino 142281, Russia}
\author{S.~Mioduszewski}\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{D.~Mishra}\affiliation{National Institute of Science Education and Research, HBNI, Jatni 752050, India}
\author{S.~Mizuno}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{B.~Mohanty}\affiliation{National Institute of Science Education and Research, HBNI, Jatni 752050, India}
\author{M.~M.~Mondal}\affiliation{Institute of Physics, Bhubaneswar 751005, India}
\author{D.~A.~Morozov}\affiliation{Institute of High Energy Physics, Protvino 142281, Russia}
\author{M.~K.~Mustafa}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{Md.~Nasim}\affiliation{University of California, Los Angeles, California 90095}
\author{T.~K.~Nayak}\affiliation{Variable Energy Cyclotron Centre, Kolkata 700064, India}
\author{J.~M.~Nelson}\affiliation{University of California, Berkeley, California 94720}
\author{M.~Nie}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{G.~Nigmatkulov}\affiliation{National Research Nuclear University MEPhI, Moscow 115409, Russia}
\author{T.~Niida}\affiliation{Wayne State University, Detroit, Michigan 48201}
\author{L.~V.~Nogach}\affiliation{Institute of High Energy Physics, Protvino 142281, Russia}
\author{T.~Nonaka}\affiliation{University of Tsukuba, Tsukuba, Ibaraki, Japan,305-8571}
\author{S.~B.~Nurushev}\affiliation{Institute of High Energy Physics, Protvino 142281, Russia}
\author{G.~Odyniec}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{A.~Ogawa}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{K.~Oh}\affiliation{Pusan National University, Pusan 46241, Korea}
\author{V.~A.~Okorokov}\affiliation{National Research Nuclear University MEPhI, Moscow 115409, Russia}
\author{D.~Olvitt~Jr.}\affiliation{Temple University, Philadelphia, Pennsylvania 19122}
\author{B.~S.~Page}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{R.~Pak}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{Y.~Pandit}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\author{Y.~Panebratsev}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{B.~Pawlik}\affiliation{Institute of Nuclear Physics PAN, Cracow 31-342, Poland}
\author{H.~Pei}\affiliation{Central China Normal University, Wuhan, Hubei 430079}
\author{C.~Perkins}\affiliation{University of California, Berkeley, California 94720}
\author{J.~Pluta}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{K.~Poniatowska}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{J.~Porter}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{M.~Posik}\affiliation{Temple University, Philadelphia, Pennsylvania 19122}
\author{N.~K.~Pruthi}\affiliation{Panjab University, Chandigarh 160014, India}
\author{M.~Przybycien}\affiliation{AGH University of Science and Technology, FPACS, Cracow 30-059, Poland}
\author{J.~Putschke}\affiliation{Wayne State University, Detroit, Michigan 48201}
\author{A.~Quintero}\affiliation{Temple University, Philadelphia, Pennsylvania 19122}
\author{S.~Ramachandran}\affiliation{University of Kentucky, Lexington, Kentucky 40506-0055}
\author{R.~L.~Ray}\affiliation{University of Texas, Austin, Texas 78712}
\author{R.~Reed}\affiliation{Lehigh University, Bethlehem, Pennsylvania 18015}
\author{M.~J.~Rehbein}\affiliation{Creighton University, Omaha, Nebraska 68178}
\author{H.~G.~Ritter}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{J.~B.~Roberts}\affiliation{Rice University, Houston, Texas 77251}
\author{O.~V.~Rogachevskiy}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{J.~L.~Romero}\affiliation{University of California, Davis, California 95616}
\author{J.~D.~Roth}\affiliation{Creighton University, Omaha, Nebraska 68178}
\author{L.~Ruan}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{J.~Rusnak}\affiliation{Nuclear Physics Institute AS CR, 250 68 Prague, Czech Republic}
\author{O.~Rusnakova}\affiliation{Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\author{N.~R.~Sahoo}\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{P.~K.~Sahu}\affiliation{Institute of Physics, Bhubaneswar 751005, India}
\author{S.~Salur}\affiliation{Rutgers University, Piscataway, New Jersey 08854}
\author{J.~Sandweiss}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{M.~Saur}\affiliation{Nuclear Physics Institute AS CR, 250 68 Prague, Czech Republic}
\author{J.~Schambach}\affiliation{University of Texas, Austin, Texas 78712}
\author{A.~M.~Schmah}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{W.~B.~Schmidke}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{N.~Schmitz}\affiliation{Max-Planck-Institut fur Physik, Munich 80805, Germany}
\author{B.~R.~Schweid}\affiliation{State University of New York, Stony Brook, New York 11794}
\author{J.~Seger}\affiliation{Creighton University, Omaha, Nebraska 68178}
\author{M.~Sergeeva}\affiliation{University of California, Los Angeles, California 90095}
\author{R.~ Seto}\affiliation{University of California, Riverside, California 92521}
\author{P.~Seyboth}\affiliation{Max-Planck-Institut fur Physik, Munich 80805, Germany}
\author{N.~Shah}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{E.~Shahaliev}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{P.~V.~Shanmuganathan}\affiliation{Lehigh University, Bethlehem, Pennsylvania 18015}
\author{M.~Shao}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{W.~Q.~Shen}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{Z.~Shi}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{S.~S.~Shi}\affiliation{Central China Normal University, Wuhan, Hubei 430079}
\author{Q.~Y.~Shou}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{E.~P.~Sichtermann}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{R.~Sikora}\affiliation{AGH University of Science and Technology, FPACS, Cracow 30-059, Poland}
\author{M.~Simko}\affiliation{Nuclear Physics Institute AS CR, 250 68 Prague, Czech Republic}
\author{S.~Singha}\affiliation{Kent State University, Kent, Ohio 44242}
\author{M.~J.~Skoby}\affiliation{Indiana University, Bloomington, Indiana 47408}
\author{D.~Smirnov}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{N.~Smirnov}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{W.~Solyst}\affiliation{Indiana University, Bloomington, Indiana 47408}
\author{P.~Sorensen}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{H.~M.~Spinka}\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}
\author{B.~Srivastava}\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{T.~D.~S.~Stanislaus}\affiliation{Valparaiso University, Valparaiso, Indiana 46383}
\author{M.~Strikhanov}\affiliation{National Research Nuclear University MEPhI, Moscow 115409, Russia}
\author{B.~Stringfellow}\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{A.~A.~P.~Suaide}\affiliation{Universidade de Sao Paulo, Sao Paulo, Brazil, 05314-970}
\author{T.~Sugiura}\affiliation{University of Tsukuba, Tsukuba, Ibaraki, Japan,305-8571}
\author{M.~Sumbera}\affiliation{Nuclear Physics Institute AS CR, 250 68 Prague, Czech Republic}
\author{B.~Summa}\affiliation{Pennsylvania State University, University Park, Pennsylvania 16802}
\author{Y.~Sun}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{X.~Sun}\affiliation{Central China Normal University, Wuhan, Hubei 430079}
\author{X.~M.~Sun}\affiliation{Central China Normal University, Wuhan, Hubei 430079}
\author{B.~Surrow}\affiliation{Temple University, Philadelphia, Pennsylvania 19122}
\author{D.~N.~Svirida}\affiliation{Alikhanov Institute for Theoretical and Experimental Physics, Moscow 117218, Russia}
\author{Z.~Tang}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{A.~H.~Tang}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{A.~Taranenko}\affiliation{National Research Nuclear University MEPhI, Moscow 115409, Russia}
\author{T.~Tarnowsky}\affiliation{Michigan State University, East Lansing, Michigan 48824}
\author{A.~Tawfik}\affiliation{World Laboratory for Cosmology and Particle Physics (WLCAPP), Cairo 11571, Egypt}
\author{J.~Th{\"a}der}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{J.~H.~Thomas}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{A.~R.~Timmins}\affiliation{University of Houston, Houston, Texas 77204}
\author{D.~Tlusty}\affiliation{Rice University, Houston, Texas 77251}
\author{T.~Todoroki}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{M.~Tokarev}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{S.~Trentalange}\affiliation{University of California, Los Angeles, California 90095}
\author{R.~E.~Tribble}\affiliation{Texas A\&M University, College Station, Texas 77843}
\author{P.~Tribedy}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{S.~K.~Tripathy}\affiliation{Institute of Physics, Bhubaneswar 751005, India}
\author{B.~A.~Trzeciak}\affiliation{Czech Technical University in Prague, FNSPE, Prague, 115 19, Czech Republic}
\author{O.~D.~Tsai}\affiliation{University of California, Los Angeles, California 90095}
\author{T.~Ullrich}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{D.~G.~Underwood}\affiliation{Argonne National Laboratory, Argonne, Illinois 60439}
\author{I.~Upsal}\affiliation{Ohio State University, Columbus, Ohio 43210}
\author{G.~Van~Buren}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{G.~van~Nieuwenhuizen}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{A.~N.~Vasiliev}\affiliation{Institute of High Energy Physics, Protvino 142281, Russia}
\author{F.~Videb{\ae}k}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{S.~Vokal}\affiliation{Joint Institute for Nuclear Research, Dubna, 141 980, Russia}
\author{S.~A.~Voloshin}\affiliation{Wayne State University, Detroit, Michigan 48201}
\author{A.~Vossen}\affiliation{Indiana University, Bloomington, Indiana 47408}
\author{Y.~Wang}\affiliation{Tsinghua University, Beijing 100084}
\author{F.~Wang}\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{G.~Wang}\affiliation{University of California, Los Angeles, California 90095}
\author{Y.~Wang}\affiliation{Central China Normal University, Wuhan, Hubei 430079}
\author{G.~Webb}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{J.~C.~Webb}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{L.~Wen}\affiliation{University of California, Los Angeles, California 90095}
\author{G.~D.~Westfall}\affiliation{Michigan State University, East Lansing, Michigan 48824}
\author{H.~Wieman}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{S.~W.~Wissink}\affiliation{Indiana University, Bloomington, Indiana 47408}
\author{R.~Witt}\affiliation{United States Naval Academy, Annapolis, Maryland 21402}
\author{Y.~Wu}\affiliation{Kent State University, Kent, Ohio 44242}
\author{Z.~G.~Xiao}\affiliation{Tsinghua University, Beijing 100084}
\author{W.~Xie}\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{G.~Xie}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{Y.~F.~Xu}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{J.~Xu}\affiliation{Central China Normal University, Wuhan, Hubei 430079}
\author{N.~Xu}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{Z.~Xu}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{Q.~H.~Xu}\affiliation{Shandong University, Jinan, Shandong 250100}
\author{Q.~Yang}\affiliation{Shandong University, Jinan, Shandong 250100}
\author{Y.~Yang}\affiliation{National Cheng Kung University, Tainan 70101 }
\author{C.~Yang}\affiliation{Shandong University, Jinan, Shandong 250100}
\author{S.~Yang}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{Z.~Ye}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\author{Z.~Ye}\affiliation{University of Illinois at Chicago, Chicago, Illinois 60607}
\author{L.~Yi}\affiliation{Yale University, New Haven, Connecticut 06520}
\author{K.~Yip}\affiliation{Brookhaven National Laboratory, Upton, New York 11973}
\author{I.~-K.~Yoo}\affiliation{Pusan National University, Pusan 46241, Korea}
\author{N.~Yu}\affiliation{Central China Normal University, Wuhan, Hubei 430079}
\author{H.~Zbroszczyk}\affiliation{Warsaw University of Technology, Warsaw 00-661, Poland}
\author{W.~Zha}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{J.~Zhang}\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\author{S.~Zhang}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{X.~P.~Zhang}\affiliation{Tsinghua University, Beijing 100084}
\author{Y.~Zhang}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{J.~Zhang}\affiliation{Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000}
\author{Z.~Zhang}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{S.~Zhang}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{J.~B.~Zhang}\affiliation{Central China Normal University, Wuhan, Hubei 430079}
\author{J.~Zhao}\affiliation{Purdue University, West Lafayette, Indiana 47907}
\author{C.~Zhong}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{L.~Zhou}\affiliation{University of Science and Technology of China, Hefei, Anhui 230026}
\author{C.~Zhou}\affiliation{Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\author{Z.~Zhu}\affiliation{Shandong University, Jinan, Shandong 250100}
\author{X.~Zhu}\affiliation{Tsinghua University, Beijing 100084}
\author{M.~Zyzak}\affiliation{Frankfurt Institute for Advanced Studies FIAS, Frankfurt 60438, Germany}
\collaboration{STAR Collaboration}\noaffiliation
